Preflight Characterization of the BLAST-TNG Receiver and Detector Arrays

The Next Generation Balloon-borne Large Aperture Submillimeter Telescope (BLAST-TNG) is a submillimeter mapping experiment planned for a 28 day long-duration balloon (LDB) flight from McMurdo Station, Antarctica during the 2018-2019 season. BLAST-TNG will detect submillimeter polarized interstellar dust emission, tracing magnetic fields in galactic molecular clouds. BLAST-TNG will be the first polarimeter with the sensitivity and resolution to probe the $\sim$0.1 parsec-scale features that are critical to understanding the origin of structures in the interstellar medium. BLAST-TNG features three detector arrays operating at wavelengths of 250, 350, and 500 $\mu$m (1200, 857, and 600 GHz) comprised of 918, 469, and 272 dual-polarization pixels, respectively. Each pixel is made up of two crossed microwave kinetic inductance detectors (MKIDs). These arrays are cooled to 275 mK in a cryogenic receiver. Each MKID has a different resonant frequency, allowing hundreds of resonators to be read out on a single transmission line. This inherent ability to be frequency-domain multiplexed simplifies the cryogenic readout hardware, but requires careful optical testing to map out the physical location of each resonator on the focal plane. Receiver-level optical testing was carried out using both a cryogenic source mounted to a movable xy-stage with a shutter, and a beam-filling, heated blackbody source able to provide a 10-50 $^\circ$C temperature chop. The focal plane array noise properties, responsivity, polarization efficiency, instrumental polarization were measured. We present the preflight characterization of the BLAST-TNG cryogenic system and array-level optical testing of the MKID detector arrays in the flight receiver.

==> Future_Work.tex <==
\section{Future Work}
\label{section:future}  % \label{} allows reference to this section

==> ScienceGoals.tex <==
\section{Science Goals}
\label{section:science}

For decades, there has been much debate as to why star formation is such an inefficient process, and why observed star formation rates in molecular clouds are many times lower than that predicted by simple gravitation collapse models. Key to resolving this debate is understanding the relative contributions of gravity, supersonic turbulence, and magnetic fields to the early stages of star formation. Recent data from the \emph{Herschel} satellite have shown that the interstellar medium (ISM) is pervaded by long, gravitationally-bound filamentary structures \cite{herschel} which are rich with dense prestellar cores. Data from polarimeters like \emph{Planck} and BLAST-Pol \cite{planckFilaments,blastpol} have shown that the magnetic fields are highly coherent around these filaments, and tend to be aligned perpendicular to the filament direction. This suggests that magnetic fields play an important role in the initial formation of these filaments, and that these filaments are persistent structures which draw in mass from the diffuse regions of the cloud along the magnetic field lines. 

The ISM is filled with tiny (0.1-10 $\mu$m), irregularly-shaped, silicate and carbonaceous smoke-like dust particles. Though they account for less than one percent of the mass of the large gas clouds in the ISM, this dust dominates the thermal emission. In the presence of large-scale magnetic fields, these grains align preferentially with their long axis perpendicular to the direction of the field, through a process of radiative torques \cite{lazarian}. Because of this grain alignment, the magnetic field morphology of the cloud can be traced observationally by mapping the polarization of thermal emission of dusty clouds at submillimeter wavelengths. 

The primary science goal of BLAST-TNG is to map the polarized thermal emission from galactic interstellar dust around star-forming regions and in the diffuse interstellar medium (ISM). These maps will yield millions of polarization vectors on the sky, allowing us to explore correlations between the magnetic field dispersion, polarization fraction, cloud temperature and column density. Quantifying the relationships between these variables over a large sample of clouds will yield testable relationships which can be fed back into numerical simulations. Combining the BLAST-TNG data with numerical models will give unprecedented insight into the interplay between gravitational, turbulent and magnetic field contributions to star and cloud formation, as well as the physics of grain alignment and mass flow within the clouds.

BLAST-TNG is also a powerful instrument for cosmic microwave background (CMB) foreground characterization and will be able to make the deepest maps to date of the dust emission in the darkest patches of the sky observed by state of the art CMB polarization experiments.  Because BLAST-TNG has focal planes with thousands of detectors, and because the intensity of thermal dust signal rises steeply as a function of frequency in the submillimeter, the BLAST-TNG maps of this region will have higher fidelity than the highest frequency \emph{Planck} maps at 353 GHz. 




